Ultrafast all-optical switching in nonlinear 3R-MoS$_2$ van der Waals metasurfaces

Second-order nonlinear optical processes are fundamental to photonics, spectroscopy, and information technologies, with material platforms playing a pivotal role in advancing these applications. Here, we demonstrate the exceptional nonlinear optical properties of the van der Waals crystal 3R-MoS$_2$, a rhombohedral polymorph exhibiting high second-order optical susceptibility ($\chi^{(2)}$) and remarkable second-harmonic generation (SHG) capabilities. By designing high quality factor resonances in 3R-MoS$_2$ metasurfaces supporting quasi-bound states in the continuum (qBIC), we first demonstrate SHG efficiency enhancement exceeding 10$^2$. Additionally, by using degenerate pump-probe spectroscopy, we harness the C$_{3v}$ system's symmetry to realize ultrafast SHG polarization switching with near-unity modulation depth. The operation speeds are limited only by the excitation pulse duration, allowing its characterization via the nonlinear autocorrelation function. These findings establish 3R-MoS$_2$ as a transformative platform for nanoscale nonlinear optics, offering large conversion efficiencies and ultrafast response times for advanced pulse measurement devices, integrated photonics, and quantum technologies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
